H.E.S.S. follow-up observations of Binary Black Hole Coalescence events during the second and third Gravitational Waves observing runs of Advanced LIGO and Advanced Virgo

We report on the observations of four well-localized binary black hole (BBH) mergers by the High Energy Stereoscopic System (H.E.S.S.) during the second and third observing runs of Advanced LIGO and Advanced Virgo, O2 and O3. H.E.S.S. can observe $\mathrm{20\,deg^2}$ of the sky at a time and follows up gravitational-wave (GW) events by ``tiling'' localization regions to maximize the covered localization probability. During O2 and O3, H.E.S.S. observed large portions of the localization regions, between 35\% and 75\%, for four BBH mergers (GW170814, GW190512\_180714, GW190728\_064510, and S200224ca). For these four GW events, we find no significant signal from a pointlike source in any of the observations, and set upper limits on the very high energy ($>$100 GeV) $\gamma$-ray emission. The 1-10 TeV isotropic luminosity of these GW events is below $10^{45}$ erg s$^{-1}$ at the times of the H.E.S.S. observations, around the level of the low-luminosity GRB 190829A. Assuming no changes are made to how follow-up observations are conducted, H.E.S.S. can expect to observe over 60 GW events per year in the fourth GW observing run, O4, of which eight would be observable with minimal latency.

==> authors.tex <==
H.~Abdalla$^{1}$,
F.~Aharonian$^{2,3,4}$,
F.~Ait~Benkhali$^{3}$,
E.O.~Ang\"uner$^{5}$,
C.~Arcaro$^{6}$,
C.~Armand$^{7}$,
T.~Armstrong$^{8}$,
H.~Ashkar$^{9}$,
M.~Backes$^{1,6}$,
V.~Baghmanyan$^{10}$,
V.~Barbosa~Martins$^{11}$,
A.~Barnacka$^{12}$,
M.~Barnard$^{6}$,
Y.~Becherini$^{13}$,
D.~Berge$^{11}$,
K.~Bernl\"ohr$^{3}$,
B.~Bi$^{14}$,
E.~Bissaldi$^{15,16}$,
M.~B\"ottcher$^{6}$,
C.~Boisson$^{17}$,
J.~Bolmont$^{18}$,
M.~de~Bony~de~Lavergne$^{7}$,
M.~Breuhaus$^{3}$,
F.~Brun$^{9}$,
P.~Brun$^{9}$,
M.~Bryan$^{19}$,
M.~B\"{u}chele$^{20}$,
T.~Bulik$^{21}$,
T.~Bylund$^{13}$,
S.~Caroff$^{7}$,
A.~Carosi$^{7}$,
S.~Casanova$^{3,10}$,
T.~Chand$^{6}$,
S.~Chandra$^{6}$,
A.~Chen$^{22}$,
G.~Cotter$^{8}$,
M.~Cury{\l}o$^{21}$,
J.~Damascene~Mbarubucyeye$^{11}$,
I.D.~Davids$^{1}$,
J.~Davies$^{8}$,
C.~Deil$^{3}$,
J.~Devin$^{23}$,
L.~Dirson$^{24}$,
A.~Djannati-Ata\"i$^{23}$,
A.~Dmytriiev$^{17}$,
A.~Donath$^{3}$,
V.~Doroshenko$^{14}$,
L.~Dreyer$^{6}$,
C.~Duffy$^{25}$,
J.~Dyks$^{26}$,
K.~Egberts$^{27}$,
F.~Eichhorn$^{20}$,
S.~Einecke$^{28}$,
G.~Emery$^{18}$,
J.-P.~Ernenwein$^{5}$,
K.~Feijen$^{28}$,
S.~Fegan$^{29}$,
A.~Fiasson$^{7}$,
G.~Fichet~de~Clairfontaine$^{17}$,
G.~Fontaine$^{29}$,
S.~Funk$^{20}$,
M.~F\"u{\ss}ling$^{11}$,
S.~Gabici$^{23}$,
Y.A.~Gallant$^{30}$,
G.~Giavitto$^{11}$,
L.~Giunti$^{9,23}$,
D.~Glawion$^{20}$,
J.F.~Glicenstein$^{9}$,
M.-H.~Grondin$^{31}$,
J.~Hahn$^{3}$,
M.~Haupt$^{11}$,
G.~Hermann$^{3}$,
J.A.~Hinton$^{3}$,
W.~Hofmann$^{3}$,
C.~Hoischen$^{27}$,
T.~L.~Holch$^{11}$,
M.~Holler$^{32}$,
M.~H\"{o}rbe$^{8}$,
D.~Horns$^{24}$,
D.~Huber$^{32}$,
M.~Jamrozy$^{12}$,
D.~Jankowsky$^{20}$,
F.~Jankowsky$^{33}$,
A.~Jardin-Blicq$^{3}$,
V.~Joshi$^{20}$,
I.~Jung-Richardt$^{20}$,
E.~Kasai$^{1}$,
M.A.~Kastendieck$^{24}$,
K.~Katarzy{\'n}ski$^{34}$,
U.~Katz$^{20}$,
D.~Khangulyan$^{35}$,
B.~Kh\'elifi$^{23}$,
S.~Klepser$^{11}$,
W.~Klu\'{z}niak$^{26}$,
Nu.~Komin$^{22}$,
R.~Konno$^{11}$,
K.~Kosack$^{9}$,
D.~Kostunin$^{11}$,
M.~Kreter$^{6}$,
G.~Lamanna$^{7}$,
A.~Lemi\`ere$^{23}$,
M.~Lemoine-Goumard$^{31}$,
J.-P.~Lenain$^{18}$,
F.~Leuschner$^{14}$,
C.~Levy$^{18}$,
T.~Lohse$^{36}$,
I.~Lypova$^{11}$,
J.~Mackey$^{2}$,
J.~Majumdar$^{11}$,
D.~Malyshev$^{14}$,
D.~Malyshev$^{20}$,
V.~Marandon$^{3}$,
P.~Marchegiani$^{22}$,
A.~Marcowith$^{30}$,
A.~Mares$^{31}$,
G.~Mart\'i-Devesa$^{32}$,
R.~Marx$^{33,3}$,
G.~Maurin$^{7}$,
P.J.~Meintjes$^{37}$,
M.~Meyer$^{20}$,
A.~Mitchell$^{3}$,
R.~Moderski$^{26}$,
L.~Mohrmann$^{20}$,
A.~Montanari$^{9}$,
C.~Moore$^{25}$,
P.~Morris$^{8}$,
E.~Moulin$^{9}$,
J.~Muller$^{29}$,
T.~Murach$^{11}$,
K.~Nakashima$^{20}$,
A.~Nayerhoda$^{10}$,
M.~de~Naurois$^{29}$,
H.~Ndiyavala$^{6}$,
J.~Niemiec$^{10}$,
L.~Oakes$^{36}$,
P.~O'Brien$^{25}$,
H.~Odaka$^{38}$,
S.~Ohm$^{11}$,
L.~Olivera-Nieto$^{3}$,
E.~de~Ona~Wilhelmi$^{11}$,
M.~Ostrowski$^{12}$,
S.~Panny$^{32}$,
M.~Panter$^{3}$,
R.D.~Parsons$^{36}$,
G.~Peron$^{3}$,
B.~Peyaud$^{9}$,
Q.~Piel$^{7}$,
S.~Pita$^{23}$,
V.~Poireau$^{7}$,
A.~Priyana~Noel$^{12}$,
D.A.~Prokhorov$^{19}$,
H.~Prokoph$^{11}$,
G.~P\"uhlhofer$^{14}$,
M.~Punch$^{13,23}$,
A.~Quirrenbach$^{33}$,
S.~Raab$^{20}$,
R.~Rauth$^{32}$,
P.~Reichherzer$^{9}$,
A.~Reimer$^{32}$,
O.~Reimer$^{32}$,
Q.~Remy$^{3}$,
M.~Renaud$^{30}$,
F.~Rieger$^{3}$,
L.~Rinchiuso$^{9}$,
C.~Romoli$^{3}$,
G.~Rowell$^{28}$,
B.~Rudak$^{26}$,
E.~Ruiz-Velasco$^{3}$,
V.~Sahakian$^{39}$,
S.~Sailer$^{3}$,
H.~Salzmann$^{14}$,
D.A.~Sanchez$^{7}$,
A.~Santangelo$^{14}$,
M.~Sasaki$^{20}$,
M.~Scalici$^{14}$,
J.~Sch\"afer$^{20}$,
F.~Sch\"ussler$^{9}$,
H.M.~Schutte$^{6}$,
U.~Schwanke$^{36}$,
M.~Seglar-Arroyo$^{9}$,
M.~Senniappan$^{13}$,
A.S.~Seyffert$^{6}$,
N.~Shafi$^{22}$,
J.N.S.~Shapopi$^{1}$,
K.~Shiningayamwe$^{1}$,
R.~Simoni$^{19}$,
A.~Sinha$^{23}$,
H.~Sol$^{17}$,
A.~Specovius$^{20}$,
S.~Spencer$^{8}$,
M.~Spir-Jacob$^{23}$,
{\L.}~Stawarz$^{12}$,
L.~Sun$^{19}$,
R.~Steenkamp$^{1}$,
C.~Stegmann$^{27,11}$,
S.~Steinmassl$^{3}$,
C.~Steppa$^{27}$,
T.~Takahashi$^{40}$,
T.~Tam$^{41}$,
T.~Tavernier$^{9}$,
A.M.~Taylor$^{11}$,
R.~Terrier$^{23}$,
J.~H.E.~Thiersen$^{6}$,
D.~Tiziani$^{20}$,
M.~Tluczykont$^{24}$,
L.~Tomankova$^{20}$,
M.~Tsirou$^{3}$,
R.~Tuffs$^{3}$,
Y.~Uchiyama$^{35}$,
D.J.~van~der~Walt$^{6}$,
C.~van~Eldik$^{20}$,
C.~van~Rensburg$^{1}$,
B.~van~Soelen$^{37}$,
G.~Vasileiadis$^{30}$,
J.~Veh$^{20}$,
C.~Venter$^{6}$,
P.~Vincent$^{18}$,
J.~Vink$^{19}$,
H.J.~V\"olk$^{3}$,
Z.~Wadiasingh$^{6}$,
S.J.~Wagner$^{33}$,
J.~Watson$^{8}$,
F.~Werner$^{3}$,
R.~White$^{3}$,
A.~Wierzcholska$^{10,33}$,
Yu Wun Wong$^{20}$,
A.~Yusafzai$^{20}$,
M.~Zacharias$^{6,17}$,
R.~Zanin$^{3}$,
D.~Zargaryan$^{2,4}$,
A.A.~Zdziarski$^{26}$,
A.~Zech$^{17}$,
S.J.~Zhu$^{11}$,
J.~Zorn$^{3}$,
S.~Zouari$^{23}$,
N.~\.Zywucka$^{6}$
\\\newline
1. University of Namibia, Department of Physics, Windhoek 10005, Namibia\\
2. Dublin Institute for Advanced Studies, Dublin 2, Ireland\\
3. Max-Planck-Institut f\"ur Kernphysik, D 69029 Heidelberg, Germany\\
4. High Energy Astrophysics Laboratory, Russian-Armenian University (RAU), Yerevan 0051, Armenia\\
5. Aix Marseille Universit\'e, Centre national de la recherche scientifique (CNRS)/Institut National de Physique Nucléaire et Physique des Particules (IN2P3), Centre de Physique des Particules de Marseille (CPPM), Marseille, France\\
6. Centre for Space Research, North-West University, Potchefstroom 2520, South Africa\\
7. Laboratoire d'Annecy de Physique des Particules (LAPP), Univ. Grenoble Alpes, Univ. Savoie Mont Blanc, CNRS, 74000 Annecy, France\\
8. University of Oxford, Department of Physics, Denys Wilkinson Building, Oxford OX1 3RH, UK\\
9. Institute for Research on the Fundamental Laws of the Universe (IRFU), Commissariat à l'énergie atomique (CEA), Universit\'e Paris-Saclay, F-91191 Gif-sur-Yvette, France\\
10. Instytut Fizyki J\c{a}drowej Polskiej Akademii Nauk (PAN), 31-342 Krak{\'o}w, Poland\\
11. Deutsches Elektronen-Synchrotron (DESY), D-15738 Zeuthen, Germany\\
12. Obserwatorium Astronomiczne, Uniwersytet Jagiello{\'n}ski, 30-244 Krak{\'o}w, Poland\\
13. Department of Physics and Electrical Engineering, Linnaeus University,  351 95 V\"axj\"o, Sweden\\
14. Institut f\"ur Astronomie und Astrophysik, Universit\"at T\"ubingen, D 72076 T\"ubingen, Germany\\
15. Dipartimento Interateneo di Fisica, Politecnico di Bari, 70125 Bari, Italy\\
16. Istituto Nazionale di Fisica Nucleare, Sezione di Bari, 70125 Bari, Italy\\
17. Laboratoire Univers et Th\'{e}ories, Observatoire de Paris, Universit\'{e} PSL, CNRS, Universit\'{e} de Paris, 92190 Meudon, France\\
18. Sorbonne Universit\'e, Universit\'e Paris Diderot, Sorbonne Paris Cit\'e, CNRS/IN2P3, Laboratoire de Physique Nucl\'eaire et de Hautes Energies (LPNHE), F-75252 Paris, France\\
19. Gravitation and Astroparticle Physics at the University of Amsterdam (GRAPPA), Anton Pannekoek Institute for Astronomy, University of Amsterdam, 1098 XH Amsterdam, The Netherlands\\
20. Friedrich-Alexander-Universit\"at Erlangen-N\"urnberg, Erlangen Centre for Astroparticle Physics, D 91058 Erlangen, Germany\\
21. Astronomical Observatory, The University of Warsaw, 00-478 Warsaw, Poland\\
22. School of Physics, University of the Witwatersrand, Braamfontein, Johannesburg, 2050 South Africa\\
23. Universit\'{e} de Paris, CNRS, Astroparticule et Cosmologie, F-75013 Paris, France\\
24. Universit\"at Hamburg, Institut f\"ur Experimentalphysik, D 22761 Hamburg, Germany\\
25. School of Physics and Astronomy, The University of Leicester, Leicester, LE1 7RH, United Kingdom\\
26. Nicolaus Copernicus Astronomical Center, Polish Academy of Sciences, 00-716 Warsaw, Poland\\
27. Institut f\"ur Physik und Astronomie, Universit\"at Potsdam, D 14476 Potsdam, Germany\\
28. School of Physical Sciences, University of Adelaide, Adelaide 5005, Australia\\
29. Laboratoire Leprince-Ringuet, CNRS, Institut Polytechnique de Paris, F-91128 Palaiseau, France\\
30. Laboratoire Univers et Particules de Montpellier, Universit\'e Montpellier, CNRS/IN2P3, F-34095 Montpellier Cedex 5, France\\
31. Universit\'e Bordeaux, CNRS/IN2P3, Centre d'\'Etudes Nucl\'eaires de Bordeaux Gradignan, 33175 Gradignan, France\\
32. Institut f\"ur Astro- und Teilchenphysik, Leopold-Franzens-Universit\"at Innsbruck, A-6020 Innsbruck, Austria\\
33. Landessternwarte, Universit\"at Heidelberg, K\"onigstuhl, D 69117 Heidelberg, Germany\\
34. Institute of Astronomy, Faculty of Physics, Astronomy and Informatics, Nicolaus Copernicus University, 87-100 Torun, Poland\\
35. Department of Physics, Rikkyo University, Toshima-ku, Tokyo 171-8501, Japan\\
36. Institut f\"ur Physik, Humboldt-Universit\"at zu Berlin, D 12489 Berlin, Germany\\
37. Department of Physics, University of the Free State, Bloemfontein 9300, South Africa\\
38. Department of Physics, The University of Tokyo, Bunkyo-ku, Tokyo 113-0033, Japan\\
39. Yerevan Physics Institute, 375036 Yerevan, Armenia\\
40. Kavli Institute for the Physics and Mathematics of the Universe (World Premier International Research Center Initiative (WPI)), The University of Tokyo Institutes for Advanced Study (UTIAS), The University of Tokyo, Kashiwa, Chiba, 277-8583, Japan\\
41. School of Physics and Astronomy, Sun Yat Sen University, Guangzhou 510275, People’s Republic of China\\
